An Ontology-Enabled Approach For User-Centered and Knowledge-Enabled Explanations of AI Systems

Explainable Artificial Intelligence (AI) focuses on helping humans understand the working of AI systems or their decisions and has been a cornerstone of AI for decades. Recent research in explainability has focused on explaining the workings of AI models or model explainability. There have also been several position statements and review papers detailing the needs of end-users for user-centered explainability but fewer implementations. Hence, this thesis seeks to bridge some gaps between model and user-centered explainability. We create an explanation ontology (EO) to represent literature-derived explanation types via their supporting components. We implement a knowledge-augmented question-answering (QA) pipeline to support contextual explanations in a clinical setting. Finally, we are implementing a system to combine explanations from different AI methods and data modalities. Within the EO, we can represent fifteen different explanation types, and we have tested these representations in six exemplar use cases. We find that knowledge augmentations improve the performance of base large language models in the contextualized QA, and the performance is variable across disease groups. In the same setting, clinicians also indicated that they prefer to see actionability as one of the main foci in explanations. In our explanations combination method, we plan to use similarity metrics to determine the similarity of explanations in a chronic disease detection setting. Overall, through this thesis, we design methods that can support knowledge-enabled explanations across different use cases, accounting for the methods in today's AI era that can generate the supporting components of these explanations and domain knowledge sources that can enhance them.

==> tex_chapters/studyresults.tex <==

% \todotip[DG]{Lead}
% \todotip[Dan]{Move some of these to methods.}

% We conducted sessions individually with four clinicians in our expert panel to understand whether the explanations we support that provide contextual explanations around the patient, their predicted risk, and the explanations of their risk, were helpful in clinical practice. We started by familiarizing each clinician with the different sections of the risk-prediction dashboard.  We then presented the dashboard as it would appear for a series of different simulated patients,  loosely based on actual patients with certain details modified or obscured. We asked the panel members to imagine that they were preparing to treat this patient who was new to them.  We navigated through the dashboard as instructed by the subjects, opening sections or clicking on items as they requested.  We asked the clinicians to speak aloud as they were working with the dashboard.  We also probed about the relevance and usefulness of the different sections of the dashboard and the specific content shown in them.  We asked if there was other information they would have liked to have had, or questions they would want answered. Sessions were recorded and transcribed. 

% \todotip[Dan]{Keep in results.}


% T1: connection to patient data
% T2: Highlight actionability
% T3: connections to external knowledge
% T4: Clinical value of explanations and contextualizations



% We had two expert panel sessions during the development of our pipeline, one at the beginning while we were designing prototypes for the explanations powered AI tools trying to understand the needs for such tools~\cite{dan2020designing} and another when we had the explanations that support contextualizations, integrated into the risk-prediction dashboard. We received similar feedback from clinicians during both of these sessions, and we report a combined list of themes resulting from thematic analyses of these sessions. These themes indicate the areas that clinicians prioritize and where AI tools' support would be appreciated. 

%Add to where clinicians were seeking the most support to, i.e., we wanted to validate the use of guidelines 
